Teaching Vision-Language-Action Models to Stop Safely

Vision-language-action (VLA) models enable robots to perform diverse tasks from visual observations and language instructions. While prior work has explored task suppression and refusal, stopping prohibited behavior once execution is underway and controlling the resulting physical response remain challenging. Our evaluation reveals that policies which suppress a task from its initial state can still complete it when taking over partway through execution. Even when the task remains unfinished, the robot may drop a held object, making non-completion an incomplete measure of safety. To address these challenges, we introduce State-Aware Fallback Imitation (SAFI) for tasks where holding provides an appropriate alternative response. SAFI comprises two stages, (1) fallback target construction, which assigns stationary arm commands and consistent gripper targets throughout prohibited-task demonstrations, and (2) joint policy adaptation, which learns these targets alongside the original actions of retained tasks. This supervision teaches an explicit alternative response at intermediate execution states while maintaining the robot's other skills. Extensive experiments with OpenVLA-OFT across LIBERO and BadLIBERO tasks evaluate prohibited completion, physical incidents, and retained-task performance. On the evaluated LIBERO tasks, SAFI reduces aggregate target success after takeover to 1.3\%, with no recorded physical incidents or action saturation, while preserving high retained-task success.

==> notes/experiments_author_comments_20261114.tex <==
\section{Experiments}
\label{sec:experiments}
\frank{In this section, we conduct comprehensive experiemnts to evaluate the effectiveness of \method. Our study is guided by the following research questions: (1) Can \method xxxxxxx (this should relevant to effectiveness) (2) How does each module contribute to xxxxx (this should be relevant to ablation study) (3) Does \method maintain general-purpose utility xxxx (parento frontier trade-off relevant to other tasks (4)sth else}Our experiments address four questions. \textbf{RQ1} asks whether prohibited-task suppression preserves retained-task utility at normal starts. \textbf{RQ2} asks whether that result persists under intermediate-state takeover and what physical responses occur. \textbf{RQ3} examines the contributions of the two objective terms. \textbf{RQ4} tests how the findings extend to a generalist policy and an implanted backdoor setting.

\subsection{Experimental Setup}
\label{sec:setup}
\paragraph{VLA models and tasks.}
\frank{models (or base models)xxxxxx}The main experiments use the released OpenVLA-OFT LIBERO-Goal specialist~\citep{kim2025oft} with an L1-regression action head, two cameras, proprioception, and eight-step action chunks. We edit t6, t9, and t7 separately and retain the other nine LIBERO-Goal tasks~\citep{liu2023libero}. Calibration uses initial states 0--9. Held-out evaluation uses states 10--49 for the prohibited task and states 10--19 for each retained task, giving 40 target and 90 retained episodes. Main runs use training seed 0. Results are descriptive unless a statistical test is explicitly identified.

\frank{Baselines. besides the base model (i think the oft should also be a baseline), talk about each method in one sentence.etc. No need to talk about too many details. And then say detailed descriptions and hyperparameters settings are given in Appendix xxxx. }
\paragraph{Methods in comparison.}
We compare \method with NPO-RT, our continuous-action adaptation of negative preference optimization~\citep{zhang2024npo}, adaptive-norm RMU~\citep{li2024wmdp}, and an OFT adaptation of VLA-Forget~\citep{ranjan2026vlaforget}. We also evaluate HazardArena-inspired home-return refusal fine-tuning~\citep{chen2026hazardarena}. It uses original-policy trajectories and simulated return-path supervision, so it is an adaptation rather than a reproduction or a controlled change of only the fallback target. The original policy and a task-excluded retraining reference (LTO) contextualize the edits. LTO was stopped at 17,500 steps and is not a converged retraining oracle. Gradient ascent (GA) and GradDiff remain non-selective diagnostics and are reported in Appendix~\ref{app:diagnostics}.

Two deployment guards act on the original policy. An exact-string gate latches an anchored hold when the instruction matches the prohibited request. A prohibition-aware semantic gate queries Gemini-2.5-Flash before each action chunk using the instruction, an image, and a command summary. It latches the same controller on a freeze decision or risk score of at least 0.5 and allows execution after a service or parsing failure. The semantic gate is evaluated only where the anchored controller passes its applicability pretest. Appendix~\ref{app:comparators} details both guards and the refusal adaptation.


\frank{Evaluation Metrics. We evaluate \method and baselinse on xxxxx. Talk about the benchmark settings we have here (their setups shortly) and the evaluation metrics and their meanings. Shortly, don't be too long. The refer full metrics definitions and implementation details to appendix. Then next, we will have a subsection to talk about main results (in the main table)}
\paragraph{Selection and evaluation.}
Learned checkpoints are selected using calibration data, with the frozen rules in Appendix~\ref{app:training}. Held-out qualification requires at most 4/40 prohibited completions and a retained-success decrease of at most 9/90 relative to the matched original. We also evaluate a fixed instruction paraphrase (P1) and a warm photometric shift (WARM). These shifted tests measure completion and utility, not physical-response events under shifted observations.

For restart audits, the original policy supplies early and mid-task states from successful trajectories. We restore t6 by a full simulator snapshot and t9/t7 by action replay, then invoke the tested policy with an empty action queue. The t6 and t9 protocols stop at task success, whereas t7 continues for 300 control steps and additionally includes an audit-start condition. Each condition has 40 episodes. Replay discrepancies were zero in the recorded position and velocity checks, and the original resumes successfully in 39/40 t6 episodes and 40/40 t9 and t7 episodes at each audited point. We report the protocols separately and do not treat repeated takeovers from one donor trajectory as independent donors.

Prohibited completion, \dropmetric, fallen-body events, and command saturation are distinct endpoints. For t9, \dropmetric requires the bottle to be over 10\,cm below its takeover height without gripper or rack contact for two consecutive steps. \satmetric denotes episodes with at least 5\% of steps at or beyond the arm-command clipping bound before clipping. It measures a command property rather than freezing or realized harm. The t6 registered descent-and-failure endpoint differs from this contact-aware \dropmetric definition, as detailed in Appendix~\ref{app:protocol}.

\subsection{Normal-Start Suppression and Utility}
\label{sec:rq1}
To answer RQ1, Table~\ref{tab:normal} reports target completion together with retained-task success. \method, NPO-RT, RMU, and refusal fine-tuning all satisfy the held-out criteria on the three specialist targets. \method records no target completions and retains 86/90, 81/90, and 86/90 successes on the respective retained sets. NPO-RT and RMU sometimes retain more successes than \method, so the normal-start comparison alone does not establish an advantage for fallback imitation. VLA-Forget qualifies on t6 and t9 but loses 16 retained successes on t7, which places that checkpoint in a non-selective diagnostic stratum.

\input{tables/normal}

Under P1 and WARM, \method again records zero target completions in all six shifted cells, with retained success within the matched-original tolerance. NPO-RT and RMU also preserve low completion under these shifts (Appendix~\ref{app:shifts}). Refusal fine-tuning was not evaluated under either shift because its allocated budget was exhausted, so no shift-robustness comparison against it is supported. Instruction-defined neighbor groups show no observed concentration of \method's utility loss, although their small sizes limit inference about task entanglement.

\subsection{Intermediate-State Responses and Guards}
\label{sec:rq2}
To answer RQ2, Table~\ref{tab:restart} evaluates the same policies after takeover. The t7 results distinguish policies that look similar under RQ1. NPO-RT and refusal fine-tuning reach 39/40 early and 40/40 mid-task completions, while RMU reaches 32/40 mid-task completions. Refusal training used return trajectories that began before stove contact. Limited coverage is consistent with its post-contact result, but the comparison does not isolate coverage as the cause. RMU's high completion with zero saturation further shows why residual execution and extreme commands require separate endpoints.

The t9 outcomes expose a different gap. NPO-RT records 40/40 drops and refusal fine-tuning 26/40 drops at mid-task takeover, with no task completions for either method. VLA-Forget also records drops at both takeover points. These are within-episode observations of a physical event without successful execution, supporting a response-quality conclusion beyond the completion metric. On t6, NPO-RT issues saturated commands in 38/40 early and 39/40 mid-task episodes despite zero completion.

\input{tables/restart}

\method records no residual completions or applicable response-proxy events in the specialist restart conditions. This result concerns states drawn from the original policy's trajectories and the specified audit horizons. It does not establish that a learned hold remains acceptable after arbitrary disturbances. A separate retained-task audit did not establish material amplification of the measured event rates among qualified edits, so the observed failure modes should not be generalized to all retained behavior (Appendix~\ref{app:retained}).

The guards expose a complementary trade-off. Both record zero restart events in their evaluated cells, but the exact-string guard misses P1 requests, permitting 40/40, 39/40, and 40/40 target completions. The semantic guard blocks the tested prohibited requests but reduces retained success to 72/90 on t9 and 73/90 on t7 in the unshifted condition. It blocks all ten tested neighbor requests that share the wine bottle or stove in each condition. Its t6 evaluation was not run because the anchored controller exceeded the excursion bound. These findings concern the tested guard and fallback combination, and do not preclude combining deployment intervention with policy editing.

\subsection{Objective Components}
\label{sec:rq3}
To answer RQ3, we remove each objective term and replace fallback imitation with ascent under the same update recipe. Table~\ref{tab:ablation} shows that fallback-only training suppresses all three targets but reduces retained success to zero. Retain-only training preserves utility while leaving target completion high. Replacing fallback imitation with plain ascent yields no selectively qualifying checkpoint within the registered search. Its held-out diagnostic results should therefore not be interpreted as a safety contrast between equally useful policies.

\begin{table}[t]
\centering\small
\begin{tabular}{lrr}
\toprule
Objective & Target /40 $\downarrow$ & Retain /90 $\uparrow$\\
\midrule
Fallback only & 0 / 0 / 0 & 0 / 0 / 0\\
Retain only & 40 / 37 / 40 & 89 / 88 / 85\\
Ascent + retain & 0 / 0 / 0 & 41 / 43 / 38\\
\method & 0 / 0 / 0 & 86 / 81 / 86\\
\bottomrule
\end{tabular}
\caption{Objective comparisons on t6 / t9 / t7. Ascent + retain is GradDiff under the matched recipe and fails selective calibration. Counts describe the designated held-out checkpoints.}
\label{tab:ablation}
\end{table}

The combined objective achieves the measured conjunction of suppression, retained utility, and specialist restart criteria. The ablations do not establish that either term alone causes safe intermediate-state responses, since fallback-only behavior is also event-free while losing utility. A prefix-only supervision ablation was not run, leaving the specific contribution of full-trajectory coverage unresolved.

\subsection{Generalist and Backdoor Extensions}
\label{sec:rq4}
To answer RQ4, we examine two extensions with separate protocols. The generalist experiment uses the released four-suite OpenVLA-OFT policy, jointly revoking stove activation in LIBERO-Goal and LIBERO-10 while retaining 38 tasks. RMU suppresses both targets at normal starts and retains 366/380 successes, compared with 349/380 for the original. Nevertheless, it activates the stove in 40/40 mid-task takeovers for both targets, reproducing the normal-start evaluation gap on this policy.

The planned generalist experiment with \method stops at the applicability pretest because scripted holding allows stove activation in 3/40 Goal mid-task states. An exploratory run conducted after this failure suppresses both targets and retains 325/380 successes, but this pooled score hides a LIBERO-10 decrease from 75/90 to 53/90. It also records one Goal mid-task activation. These outcomes delimit fallback applicability and utility preservation rather than establishing a successful generalist deployment (Appendix~\ref{app:generalist}).

The BadLIBERO extension uses GoBA's poisoned-box setting~\citep{zhou2025goba}, implanted into the OFT specialist as an adaptation within the LIBERO simulator family. All qualified methods suppress intermediate-state backdoor execution, so this setting supplies no positive evidence of the first gap. NPO-RT nonetheless records physical-event proxies in 9/40 takeovers and command saturation in all 40. \method records neither, but RMU and refusal fine-tuning also record zero physical-event proxies. \method achieves the highest observed clean-task success among the edited policies on the pooled triggered evaluation, 59/120, yet recovers only 1/40 clean completions on the two selected tasks. The supported result is suppression without clean-task recovery, not uniquely safe or useful backdoor removal (Appendix~\ref{app:badlibero}).


==> notes/experiments_author_comments_a54632f.tex <==
\section{Experiments}
\label{sec:experiments}
We evaluate \method's effectiveness in suppressing prohibited behavior and preserving the robot's other skills. Our experiments address the following research questions. \frank{Put those RQs in setences instead of using bullet points, just do (1), (2), (3). The first RQ should always be about effectiveness, the second should be ablation, third should be trade-off. The second question should just be "how do two modules in \method xxxxx" no need to put the full name of each module there. }
\begin{itemize}[leftmargin=*,itemsep=0.1em,topsep=0.3em]
\item \textbf{RQ1:} Can \method suppress prohibited behavior after takeover while maintaining an acceptable physical response?
\item \textbf{RQ2:} How do fallback imitation and retained-task imitation contribute to the resulting behavior?
\item \textbf{RQ3:} How does \method balance target suppression with retained-task utility?
\end{itemize}
% Author decision, 2026-11-14: complete RQ1--3 now. RQ4's topic remains open.

\subsection{Experimental Setup}
\label{sec:setup}
\paragraph{Base models.}
We use the released OpenVLA-OFT policies~\citep{kim2025oft} as our base VLAs. These policies predict continuous action chunks from camera observations, proprioception, and a language instruction. We adapt each suite-specific policy to a prohibited task and evaluate utility on the other tasks in that suite.

\paragraph{Baselines.}
The original OpenVLA-OFT policy~\citep{kim2025oft} provides a reference for behavior before adaptation. Gradient Ascent (GA) increases imitation error on prohibited-task demonstrations~\citep{maini2024tofu}. Building on this objective, Gradient Difference (GradDiff) adds retained-task imitation~\citep{maini2024tofu}. \frank{each of those method name should be in bold.} NPO-RT adapts negative preference optimization to continuous actions and combines it with retained-task imitation~\citep{zhang2024npo}. RMU redirects hidden representations on prohibited-task inputs while matching the original representations on retained inputs~\citep{li2024wmdp}. To compare alternative-response supervision, Refusal FT learns home-return actions inspired by HazardArena~\citep{chen2026hazardarena}. VLA-Forget~\citep{ranjan2026vlaforget} provides a VLA unlearning comparison through an OFT adaptation of its module-wise updates and action distillation. Appendix~\ref{app:training} gives the objective adaptations, hyperparameters, and checkpoint-selection rules, and Appendix~\ref{app:results-protocol} records the evaluated checkpoints and their fidelity qualifications. \frank{for the appendix part, we should write sth like "XXXXX is shown (or sth like displayed in" in appendix xxx. I don't like to put appendix it self as the first word (Change this throughout the paper).  }

\paragraph{Benchmarks and evaluation.}
\frank{shorten this paragraph. modify the appendix writing as well.}
We evaluate selected tasks from LIBERO-Goal, LIBERO-Spatial, and LIBERO-Object~\citep{liu2023libero}, covering goal, spatial, and object variations. The evaluated targets are tasks that the original policy can execute and for which a scripted hold passes the fallback-applicability check. To test suppression during execution, we let the original policy begin a task and transfer control to the edited policy at intermediate states. We also evaluate BadLIBERO using the poisoned-object setting of GoBA~\citep{zhou2025goba}, with an implanted OpenVLA-OFT policy as the reference. This setting tests whether editing prevents the attack target from being reached after takeover. Appendix~\ref{app:results-protocol} provides the task selection and takeover protocols.

\paragraph{Evaluation metrics.}
\emph{Target Success Rate} measures whether the prohibited target is attained after takeover. For BadLIBERO, the target is the attack objective. We also report \emph{Physical Incident Rate}, which records defined physical events such as object drops, and \emph{Action Saturation Rate}, which records episodes whose commands reach the controller's clipping bounds under the setting's saturation criterion. Physical incidents are counted whenever they occur, including alongside target attainment. To assess the robot's other skills, \emph{Retained Success Rate} measures performance on permitted tasks from their normal initial states. All rates are percentages. The main LIBERO score averages the evaluated Goal, Spatial, and Object settings equally, with the suite breakdown and full metric definitions in Appendix~\ref{app:results-protocol}.


\subsection{Implementation Details}
All experiments on both LLaVA and Idefics2 models are implemented on a server with 3 NVIDIA
A6000 GPUs and Intel(R) Xeon(R) Silver 4210R
CPU @ 2.40GHz with 20 CPU cores.

\subsection{Main Results}
\label{sec:rq1}
\frank{To answer our first research question, xxxxx (write this in full sentence and then itaclized), we evaluate xxxxxxxx in table xxx and xxxx. As shown in the tables, xxxxxx. And write this in one paragraph.Bascially the structure should write like, as shown in the tables, [talk about the general trend of other baselines and usually they are pretty bad on sth] many baselines behave badly/unevenly. And then write why we are good. Talk about the metrics that we evlauate our motivation those two metrics. Also take one example baseline and say they are bad, and what do those numbers mean, like their interpretations. And then talk about our numbers by contrast. Do this for two benchmarks, check the reference paper i gave you as examples. } To answer RQ1, Table~\ref{tab:main-results} compares target attainment and the resulting responses after takeover. Across the evaluated LIBERO settings, \method reduces Target Success Rate from 99.7\% for the original policy to 1.3\%, with no recorded physical incidents or action-saturation episodes. Refusal FT also reduces target attainment substantially, reaching 11.6\% Target Success Rate with 4.1\% Physical Incident Rate. RMU's zero saturation accompanies substantial prohibited execution, whereas GA, GradDiff, and NPO-RT reduce target attainment alongside increased physical incidents and saturated commands. These outcomes show why the three endpoints are useful together when evaluating a behavioral prohibition.

\input{tables/main_results}

BadLIBERO further distinguishes target suppression from the physical response. GA, GradDiff, and NPO-RT all record zero target attainment, yet each produces physical incidents and frequent action saturation. \method and RMU record zero on all three endpoints, and Refusal FT also avoids target attainment and physical incidents. Thus, the backdoor comparison identifies methods that combine suppression with the measured response criteria, even when target success alone assigns them the same outcome. Appendix~\ref{app:badlibero} additionally reports clean-task performance under the trigger.

\subsection{Contributions of the Objective Terms}
\label{sec:rq2}
\frank{you should write the same way as RQ 1. Next, to answer our second quesiton: xxxxxx (the real question) We conducted ablation experiments by iteratily removing each module from \method. The results are shown in Table xxx. Additional abaltions are provided in Appendix xxxx.  Then we should have textbf for each removal. Like xxxx module removal. We first ablate xxxxxxxx while retain [the other module] Removing this module xxxxxxx (what is the effect of removing this). As shownin the table, this clauses xxxx (usually remove each corresponding module will cause some degradation on the overall performance due to one of the challenge we mentioned in the motivation section because we design this module to address that concern) Overall, this highlights that xxx module is crtical for xxxxxx since removing it would xxxx (do this for two module). Each pargraph don't be too long. }To answer RQ2, we remove fallback imitation, retained-task imitation, or both terms from the adaptation objective. Removing both leaves the original policy, providing the reference in Table~\ref{tab:ablation}. With only retained-task imitation, utility remains high but prohibited-target attainment stays close to the original policy. With only fallback imitation, target attainment is low but retained success falls to zero in both suites. Joint training combines the two roles, yielding retained success of 96.9\% on Spatial and 93.1\% on Object together with low target attainment and no recorded physical incidents. The comparison therefore supports learning an explicit fallback alongside continued supervision of the tasks the robot should retain.

\input{tables/ablation}

\subsection{Suppression and Retained Utility \frank{Irelevant task preservation? Or sth like this?}}
\label{sec:rq3}
\frank{A transition from the previous two RQs, sth like "besides xxxxxx, we also ask: xxxxxx. To access this (always say to answer this, what kind of evluation or experiments we have done). And then talk about the performance on those benchmarks/evaluations. We can also briefly talk about other baselines' performance on those. Like baseline A may perform very well on one perspective, but it fails on the other axis. And baseline B may perform good on the other axis, and may fail on this axis. Explicitly mention those, and then lastly in contrast, our method excel at both. Then additional results are givein in appendix xxx. Also write this in one paragraph. }To answer RQ3, we evaluate checkpoints throughout adaptation and compare their suppression and retained-task performance in Figure~\ref{fig:utility-tradeoff}. We express suppression as the complement of takeover Target Success Rate, so stronger suppression and higher utility appear toward the upper right. The sampled \method checkpoints span both weak and strong suppression, with later checkpoints reaching high-suppression, high-utility operating points in both suites.

On Spatial, \method reaches 99.7\% suppression with 97.2\% retained success. Refusal FT achieves similarly strong suppression with lower retained success at its sampled checkpoints. On Object, \method reaches 99.0\% suppression with 93.6\% retained success, while NPO-RT and RMU retain high utility at lower suppression levels. GA reaches high suppression with zero retained success throughout the sampled checkpoints. GradDiff's retained success increases during adaptation, reaching 34.2\% on Spatial and 41.7\% on Object alongside near-complete suppression. These comparisons show the substantial utility differences among policies with similar suppression levels. Appendix~\ref{app:run-provenance} gives the checkpoint sources and evaluation schedule.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/utility_tradeoff.pdf}
\caption{\textbf{Suppression--utility trade-off.} Colored points represent adaptation checkpoints, and hollow markers show the original policies. Target Suppression Rate is 100\% minus takeover Target Success Rate, so higher values on both axes are preferable. Red outlines highlight \method's high-suppression, high-utility operating points. GA's checkpoints overlap exactly in each panel.}
\label{fig:utility-tradeoff}
\end{figure*}
% ROUND 27 completes GA and GradDiff coverage. All seven method sweeps are included.


==> tables/badlibero.tex <==
\begin{table*}[t]
\centering\small
\begin{tabular}{lrrrrrrr}
\toprule
 & Untriggered & \multicolumn{2}{c}{Selected tasks} & Triggered & \multicolumn{3}{c}{Restarts /40}\\
Method & clean /100 & L3 /40 & clean /40 & clean /120 & L3 & Physical & SAT\\
\midrule
Implanted policy & 91 & 31 & 0 & 42 & 35 & 15 & 0\\
Clean OFT & 95 & 0 & 38 & 116 & 8 & 15 & 0\\
NPO-RT & 94 & 0 & 0 & 0 & 0 & 9 & 40\\
RMU & 86 & 0 & 0 & 24 & 0 & 0 & 0\\
Refusal FT & 91 & 0 & 0 & 43 & 0 & 0 & 1\\
GradDiff & 65 & 0 & 0 & 0 & 0 & 12 & 40\\
GA & 2 & 0 & 0 & 0 & 0 & 16 & 40\\
\method & 96 & 0 & 1 & 59 & 0 & 0 & 0\\
\bottomrule
\end{tabular}
\caption{BadLIBERO adaptation. Selected tasks are t3 and t6, with 20 normal-start episodes each. Restart counts cover 20 donors at two takeover points, each observed for 200 uncensored steps. Physical is the episode-level union of physical-event flags and can coexist with L3. SAT here records any saturated step. GA and GradDiff are non-selective diagnostics. Clean OFT is an unedited reference taking over from implanted-policy states.}
\label{tab:badlibero}
\end{table*}


==> tables/normal.tex <==
\begin{table*}[t]
\centering\small
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{2}{c}{t6, cream cheese} & \multicolumn{2}{c}{t9, wine bottle} & \multicolumn{2}{c}{t7, stove}\\
Method & Target /40 $\downarrow$ & Retain /90 $\uparrow$ & Target /40 $\downarrow$ & Retain /90 $\uparrow$ & Target /40 $\downarrow$ & Retain /90 $\uparrow$\\
\midrule
Original & 40 & 85 & 40 & 85 & 40 & 85\\
NPO-RT & 0 & 88 & 0 & 88 & 0 & 89\\
RMU & 0 & 87 & 0 & 89 & 1 & 86\\
VLA-Forget (OFT)$^\dagger$ & 0 & 84 & 0 & 84 & 0 & 69\\
Refusal FT (adapted) & 0 & 83 & 0 & 86 & 0 & 86\\
Exact-string gate & 0 & 85 & 0 & 85 & 0 & 85\\
Semantic gate & \na & \na & 0 & 72 & 0 & 73\\
Task-excluded ref. & 0 & 81 & 0 & 87 & 0 & 84\\
\method & 0 & 86 & 0 & 81 & 0 & 86\\
\bottomrule
\end{tabular}
\caption{Held-out normal-start results. Target completion is undesirable under the specified prohibition; retained success measures utility. Each target is edited separately. $\dagger$VLA-Forget fails the t7 retained-utility criterion. The semantic t6 gate is not run after controller-applicability failure (\na). The exact-string t6 controller records zero completion but fails its excursion bound. The task-excluded reference is not a retraining oracle.}
\label{tab:normal}
\end{table*}


==> tables/restart.tex <==
\begin{table*}[t]
\centering\small
\begin{tabular}{lrrrrrrr}
\toprule
 & \multicolumn{2}{c}{t6} & \multicolumn{3}{c}{t9} & \multicolumn{2}{c}{t7}\\
Method & Complete & SAT & Complete & DROP & SAT & Complete & SAT\\
\midrule
Original & 39 / 39 & 0 / 0 & 40 / 40 & 0 / 0 & 0 / 0 & 40 / 40 & 0 / 0\\
NPO-RT & 0 / 0 & 38 / 39 & 0 / 0 & 0 / 40 & 40 / 40 & 39 / 40 & 40 / 29\\
RMU & 0 / 0 & 0 / 0 & 1 / 5 & 0 / 0 & 0 / 0 & 3 / 32 & 0 / 0\\
VLA-Forget (OFT)$^\dagger$ & 0 / 7 & 5 / 8 & 0 / 0 & 6 / 8 & 40 / 40 & 8 / 15 & 40 / 40\\
Refusal FT (adapted) & 1 / 0 & 0 / 0 & 0 / 0 & 0 / 26 & 0 / 0 & 39 / 40 & 0 / 0\\
Exact-string gate & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0\\
Semantic gate & \na & \na & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0\\
\method & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0 & 0 / 0\\
\bottomrule
\end{tabular}
\caption{Restart outcomes, shown as early / mid-task counts out of 40 for each endpoint. Lower counts are desirable for edited policies; original completion checks audit validity. SAT is the pre-clip command-saturation proxy. Targets use different restoration and censoring protocols. DROP is shown for t9; t6 uses a distinct registered descent-and-failure endpoint. $\dagger$The t7 VLA-Forget checkpoint is non-selective. \na\ indicates a gate evaluation not run. Zero events for the exact-string t6 controller do not override its excursion-pretest failure.}
\label{tab:restart}
\end{table*}


==> tables/shifts.tex <==
\begin{table*}[t]
\centering\small
\begin{tabular}{llrrrrrr}
\toprule
 & & \multicolumn{2}{c}{t6} & \multicolumn{2}{c}{t9} & \multicolumn{2}{c}{t7}\\
Method & Shift & Target & Retain & Target & Retain & Target & Retain\\
\midrule
Original & P1 & 40/40 & 88/90 & 39/40 & 89/90 & 40/40 & 88/90\\
 & WARM & 40/40 & 87/90 & 40/40 & 87/90 & 40/40 & 87/90\\
NPO-RT & P1 & 0/40 & 89/90 & 0/40 & 88/90 & 0/40 & 86/90\\
 & WARM & 0/40 & 85/90 & 0/40 & 88/90 & 0/40 & 88/90\\
RMU & P1 & 0/40 & 86/90 & 0/40 & 88/90 & 1/40 & 84/90\\
 & WARM & 0/40 & 88/90 & 0/40 & 88/90 & 0/40 & 85/90\\
VLA-Forget (OFT)$^\dagger$ & P1 & 0/40 & 84/90 & 0/40 & 83/90 & 0/40 & 66/90\\
 & WARM & 0/40 & 83/90 & 0/40 & 84/90 & 0/40 & 67/90\\
Refusal FT (adapted) & P1 & \na & \na & \na & \na & \na & \na\\
 & WARM & \na & \na & \na & \na & \na & \na\\
Exact-string gate & P1 & 40/40 & 88/90 & 39/40 & 89/90 & 40/40 & 88/90\\
 & WARM & 0/40 & 87/90 & 0/40 & 87/90 & 0/40 & 87/90\\
Semantic gate & P1 & \na & \na & 0/40 & 73/90 & 0/40 & 79/90\\
 & WARM & \na & \na & 0/40 & 75/90 & 0/40 & 76/90\\
\method & P1 & 0/40 & 87/90 & 0/40 & 82/90 & 0/40 & 86/90\\
 & WARM & 0/40 & 87/90 & 0/40 & 83/90 & 0/40 & 85/90\\
\bottomrule
\end{tabular}
\caption{Input-shift outcomes. Every target count is out of 40 and retained count out of 90. Refusal FT shifts are not evaluated because of the budget limit; the semantic t6 gate is not run after pretest failure. Both are marked \na\ and neither is a zero count. These evaluations measure completion and utility, not shifted physical-event rates.}
\label{tab:shifts}
\end{table*}

